Safe and Balanced: A Framework for Constrained Multi-Objective Reinforcement Learning

In numerous reinforcement learning (RL) problems involving safety-critical systems, a key challenge lies in balancing multiple objectives while simultaneously meeting all stringent safety constraints. To tackle this issue, we propose a primal-based framework that orchestrates policy optimization between multi-objective learning and constraint adherence. Our method employs a novel natural policy gradient manipulation method to optimize multiple RL objectives and overcome conflicting gradients between different tasks, since the simple weighted average gradient direction may not be beneficial for specific tasks' performance due to misaligned gradients of different task objectives. When there is a violation of a hard constraint, our algorithm steps in to rectify the policy to minimize this violation. We establish theoretical convergence and constraint violation guarantees in a tabular setting. Empirically, our proposed method also outperforms prior state-of-the-art methods on challenging safe multi-objective reinforcement learning tasks.

==> files_arxiv/append_alg.tex <==
\section{Algorithms}
\begin{algorithm}[ht!] 
\caption{\textbf{MOPO-CR2}: Multi-Objective Policy Optimization with Constraint-Rectification and Correlation-Reduction}
\label{alg:MOPO-CR2}
\begin{algorithmic}[1]
\STATE \textbf{Inputs}: initial parameter $\omega_0$, empty set $\mathcal{N}_0$, $k=0$.
\FOR{$t = 0, \dots,T-1$}
\STATE Policy evaluation under $\pi_{\omega_t}: \Bar{Q}_t^i(s,a) \approx Q_{\pi_{\omega_t}}^i(s,a)$  for all $ i=1,\ldots,m+p$.
\STATE Sample $(s_j, a_j) \in \mathcal{B}_t \sim \xi \cdot \pi_{\omega_t}$, compute constrain estimation $\Bar{J}_{i,\mathcal{B}_t} = \sum_{j \in \mathcal{B}_t} \rho_{j,t}\Bar{Q}_t^i(s_j,a_j) $ for all $ i=1,\ldots,m+p$, where $\rho_{j,t}$ is the weight.
\IF{$\Bar{J}_{i,\mathcal{B}_t}\leq c_i +\beta$ for all $i=m+1,\ldots,m+p$}
\STATE $k\leftarrow k+1$
\STATE Add $\omega_t$ into set $\mathcal{N}_0$.
\STATE Compute the multi-objective policy gradient $\boldsymbol{d}_k$ and the preference $\boldsymbol{\lambda}_k$: $ \left(\boldsymbol{d}_k,\boldsymbol{\lambda}_k \right) \leftarrow \textbf{CR-MOGM}(\alpha_k, \boldsymbol\lambda_{k-1})$.
\STATE Take one-step policy update: $\omega_{t+1}=\omega_{t} +\eta \boldsymbol{d}_k$.
\ELSE
\STATE Choose any $i_t\in \left\{m+1,\dots, m+p \right\}$ such that $\Bar{J}_{i_t, \mathcal{B}_t} > c_{i_t} + \beta$.
\STATE Take one-step policy update towards minimize $J_{i_t}(\omega_t)$: 
$\omega_{t+1} \leftarrow \omega_t + \eta \nabla \Bar{J}_{i_t, \mathcal{B}_t}$.
\ENDIF
\ENDFOR{}
\STATE \textbf{Outputs}: $\omega_{\text{out}}$ uniformly chosen from $\mathcal{N}_0$.
\end{algorithmic}
\end{algorithm}




==> files_arxiv/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
        \item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}


\end{enumerate}


